Variational Hyper RNN for Sequence Modeling

In this work, we propose a novel probabilistic sequence model that excels at capturing high variability in time series data, both across sequences and within an individual sequence. Our method uses temporal latent variables to capture information about the underlying data pattern and dynamically decodes the latent information into modifications of weights of the base decoder and recurrent model. The efficacy of the proposed method is demonstrated on a range of synthetic and real-world sequential data that exhibit large scale variations, regime shifts, and complex dynamics.

==> table/ablation_latent_dim_tab.tex <==


\begin{table}[htb]
    \caption{VRNN and VHRNN with same latent dimensions.}
    \label{albat_tab_2}
     \footnotesize
    \centering
    \begin{tabular}[t]{c c c c c c}
        \toprule
        Model  & Z dim. & Hidden dim. & Hyper size & Param. & FIVO \\
        \midrule
        \multirow{3}{*}{VRNN}
            & 24 & 24 & - & 23k & $-$7.04 \\ 
            & 28 & 28 & - & 31k & $-$6.99 \\
            & 32 & 32 & - & 39k & $-$6.91 \\
        \midrule
        \multirow{3}{*}{VHRNN}
            & 24 & 12 & 16 & 24k & $-$6.92 \\ 
            & 28 & 14 & 18 & 31k & $-$6.73 \\
            & 32 & 16 & 20 & 39k & $-$6.70 \\
        \bottomrule
    \end{tabular}
    \vspace{-0.2in}
\end{table}


==> table/ht_sensor_tab.tex <==



\begin{minipage}{.42\textwidth}
    \captionof{table}{Evaluation on HT Sensor dataset.}
    \label{ht_tab}
    \centering
    \vspace{0.2cm}
    \footnotesize
    \begin{tabular}[t]{cccc}
        \toprule
        Model & Z dim. & Param. & FIVO \\
        \midrule
        \multirow{5}{*}{VRNN}
            & 20  & 14k & 6.13 \\
            & 24 & 20k & 13.70 \\
            & \textbf{28}  & \textbf{27k} & \textbf{13.86} \\
            & 32 & 34k & 12.37 \\
            & 48 & 76k & 12.69 \\
        \midrule
        \multirow{4}{*}{VHRNN}
            & 12  & 16k & 8.16 \\
            & \textbf{16} & \textbf{24k} & \textbf{14.41} \\
            & 20 & 34k & 12.45 \\
            & 24 & 46k & 13.75 \\
        \bottomrule
    \end{tabular}
\end{minipage}
\quad
\begin{minipage}{.5\textwidth}
    \captionof{table}{Ablation study with different hyper network inputs}
    \label{albat_tab_1}
    \footnotesize
    \centering
    \begin{tabular}[t]{c c c c}
        \toprule
        Dataset  & Z dim. & Hyper Input & FIVO \\
        \midrule
        \multirow{6}{*}{JSB}
            & \textbf{14}  & \textbf{latent only} & \textbf{$-$6.68} \\ 
            & 14 & hidden only & $-$6.71 \\
            & 14  & latent+hidden & $-$6.76 \\
            & \textbf{32} & \textbf{latent only} & \textbf{$-$6.76} \\
            & 32 & hidden only & $-$7.03 \\
            & 32 & latent+hidden & $-$6.82 \\
        \midrule
        \multirow{3}{*}{Synthetic-\textbf{Test}}
            & 4  & latent only & $-$5.01 \\ 
            & 4 & hidden only & $-$4.79 \\
            & \textbf{4}  & \textbf{latent+hidden} & \textbf{$-$4.68} \\
        \bottomrule
    \end{tabular}
    \vspace{0.15in}
\end{minipage}

